What User Behaviors Make the Differences During the Process of Visual Analytics?

The understanding of visual analytics process can benefit visualization researchers from multiple aspects, including improving visual designs and developing advanced interaction functions. However, the log files of user behaviors are still hard to analyze due to the complexity of sensemaking and our lack of knowledge on the related user behaviors. This work presents a study on a comprehensive data collection of user behaviors, and our analysis approach with time-series classification methods. We have chosen a classical visualization application, Covid-19 data analysis, with common analysis tasks covering geo-spatial, time-series and multi-attributes. Our user study collects user behaviors on a diverse set of visualization tasks with two comparable systems, desktop and immersive visualizations. We summarize the classification results with three time-series machine learning algorithms at two scales, and explore the influences of behavior features. Our results reveal that user behaviors can be distinguished during the process of visual analytics and there is a potentially strong association between the physical behaviors of users and the visualization tasks they perform. We also demonstrate the usage of our models by interpreting open sessions of visual analytics, which provides an automatic way to study sensemaking without tedious manual annotations.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> files/temp.tex <==
We designed tasks for this study in a way that user's behavior could be logged into a file and then analysed with machine learning techniques. These tasks are carefully tailered into the application's scene to match the study's needs. We start with easy tasks and as the user goes further he or she faces harder tasks to complete. Introduction tasks include one-step questions and only invalve one domain, Choropleth, Time chart or Interaction Panel. Hard questions invalve two domains at the same time, so users have to complete two tasks at a time. Finale questions are complex and include all 3 domans. 


The proposed task for our study includes:

1- Identification: Select one or multiple regions within the choropleth to study the data value for data region, identify the region with data in a certain range, such as the maximum value.
a. Identify the data value for a country, such as France, within the choropleth.
b. identify the trend of a country, using the line charts.
c. Identify each interaction buttons -- with different attributes.
d. Identify each interaction buttons -- with different time stamps.

2. correlate: for a selected region, correlate its data to surroundings or other regions with similar data distributions.
a. find the distribution in a small neighbor.
b. find another country with similar data value.


%identify the region with data in a certain range, such as the maximum value.

3. Explore trends: explore the evolution trends of the disease over the world/regions and across time.
a. explore the trend of a country.
b. explore the trend / waves of a region (harder).
c. explore the trends / waves worldwide, region 1, region2, region 3 (Pre-selected countries for each region) (hardest).

4. Open questions (Most challenging tasks)
We expect open questions cause the users to spend more complex behavior.
Since our first 3 categories have covered all possible combinations of visual analytics, we expect the behavior sequences are mainly composed of sequences for simpler tasks, as they are on different levels of the task abstraction.




%https://www.cs.ubc.ca/labs/imager/tr/2013/MultiLevelTaskTypology/brehmer_infovis13.pdf

Task abstraction: how, why and what?
How: interaction and visualization
Why: goals of users
What: input/output pairs


%\subsection{Task Abstraction for Exploring Sensemaking Process}

We have designed a user study to collect data for exploring the sensemaking process in immersive visualization.
The goal of our study is to record data that can capture important user behaviors during the sensemaking process, so that we can later learn useful factors with machine learning.

%https://www.cs.ubc.ca/labs/imager/tr/2013/MultiLevelTaskTypology/brehmer_infovis13.pdf
Similar to the task abstraction~\cite{6634168}, which expresses complex tasks as sequences of interdependent simpler tasks, we also design tasks range from simple to complex.
This task abstraction is ``independent of domain-specific descriptions of tasks, so that useful comparisons can be made between visualization systems targeted at different application domains", so it also applies to our geo-spatial visualization.
The task abstraction work ``distinguishes why and how a visualization task is performed, and what the task inputs and outputs are".

%how, why and what?
Here's how we design our study to capture the three components of the task abstraction.

How: interaction and visualization  -- all user behaviors involving interaction (interaction with our system) and visualization (look at visualization elements)

Why: goals of users -- we give tasks to users. For simple tasks, we view the goals of the tasks as the goals of users.

What: input/output pairs -- we also record the involved data modified by user interaction.

% 
We use our immersive system.
Our proposed tasks for the study:


1. identify one value (simplest tasks): 

1a. Identify the data value for a country, such as France, with the choropleth.

1b. identify the trend of a country, with the line chart.

1c. Identify each interaction button -- choose an attribute.

1d. Identify each interaction button -- choose a time stamp.


2. correlate multiple data elements (base tasks), either in the geo-space or time/attribute-space, or between the two spaces: 

2a. find the distribution in a small neighbor (local in the geo-space).

2b. find another country with similar data value (non-local in the geo-space).
for a selected region, correlate its data to surroundings or other regions with similar data distributions.

2c. find the region with data in a certain range, such as the maximum value.

2d. find the trends of one country with three attributes/lines in the time-space.

2e. find the trends of several countries in the time-space. 


3. Explore trends (challenging tasks), explore the evolution trends of the disease over the world/regions and across time.

3a. explore the trends from all attributes for several countries.

3b. explore the worldwide trends of one attribute.



\begin{table*}
\centering
\begin{tabular}{ |p{1.5cm}||p{8cm}|p{1cm}|p{1.5cm}|p{1.3cm}|p{1.3cm}| }
 \hline
 Category Type & Task Description & Category No. & Choropleth & Time Chart & Interaction Panel\\
 \hline
 \hline
 Space & Search for a state on the choropleth  & 1 & * &  &\\
 \hline
 Space & Identify the data value based on color for a state & 2 & * &  &\\
 \hline
 Space & Find a state with a certain value from the choropleth  & 3 & * &  &\\
 \hline
 Space & Find the maximum value from the map  & 4 & * &  &\\
 \hline
 Space & Compare the data values from two states (adjacent)  & 5 & * &  &\\
 \hline
 Space & Compare the data values from two states (not-adjacent)  & 6 & * &  &\\
 \hline
 Space & Summarize the spatial data distribution from one region with multiple states  & 7 & * &  &\\
 \hline
 Space & Summarize the spatial data distribution from two regions with multiple states  & 8 & * &  &\\
 \hline
 Space & Summarize the spatial data distribution from multiple regions  & 9 & * &  &\\
 \hline
 Open & Explore a new feature of data distribution from choropleth, such as an outlier & 10 & * &  &\\
\hline

\hline
 Time & Summarize the temporal trend of one attribute for a state & 11 &  & * &\\
\hline
 Time & Summarize the temporal trends for three attributes for a state & 12 &  & * &\\
 \hline
 Time & Compare the temporal trends from two states & 13 &  & * &\\
 \hline
 Time & Compare the temporal trends from multiple states & 14 &  & * &\\
 \hline
 Open & Explore a new feature of temporal trends, such as an outlier  & 15 &  & * &\\
 \hline 

 \hline
 Interaction & Switch data attributes (voice) & 16 &  &  & *\\
 \hline
 Interaction & Switch data attributes (gesture) & 17 &  &  & *\\
 \hline
 Interaction & Adjust time selections (voice) & 18 & &  & *\\
 \hline
 Interaction & Adjust time selections (gesture) & 19 & &  & *\\
 \hline
 Interaction & Select a state (gesture) & 20 & * &  & \\
 \hline
 Interaction & Deselect a state (gesture) & 21 &  &  & * \\
 \hline
 Interaction & Clear the selected states (gesture) & 22 & * &  & \\
 \hline
 
 \hline
 Combined & Explore spatial distribution among interested states for different data attributes (two or three attributes)
 & 23 & * &  & *\\
 \hline
 Combined & Explore spatial distribution among interested states during different time ranges (at least two ranges) & 24 & * &  & *\\
 \hline
 Combined & Explore temporal trends among interested states for different data attributes & 25 &  & * & *\\
 \hline
 Combined & Explore temporal trends among interested states during different time ranges & 26 &  & * & *\\

 \hline
 Combined & Explore spatial distribution among interested states and their temporal trends & 27 & * & * &\\
% \hline
% Combined & Explore the temporal trends of countries and explore their spatial data distribution & 26 & * & * &\\
% \hline
% Open & Explore the features  & 22 & * & * & \\
 
 \hline
 Combined & Explore the spatial distribution from multiple time ranges for multiple attributes
 & 28 & * & * & * \\
 \hline
 Combined & Explore the temporal trends from multiple time range for multiple attributes
 & 29 & * & * & * \\
 \hline
 Combined & Explore the features from multiple time range for multiple attributes, such as finding outliers
 & 30 & * & * & * \\
 \hline
 Open & Explore a new data feature with the whole system & 31 & * & * & *\\
 \hline
\end{tabular}
\caption{Task Design}
\label{table:task}
\end{table*}


\subsection{Data Collection}
Data collected from HoloLens:

Basic: userIndex, taskNumber, time stamp, 

\textbf{Interaction: valueMonitorTap, valueMonitorGaze, valueMonitorVoice, valuemonitorAttribute, valuemonitorTime, valuemonitorDeselect,
objPosition.x, objPosition.y, objPosition.z, (obj name)}

User status: camera.transform.position.x, camera.transform.position.y, camera.transform.position.z,
camera.transform.forward.x, camera.transform.forward.y, camera.transform.forward.z,
camera.transform.up.x, camera.transform.up.y, camera.transform.up.z;

Vis status: selected time stamp, attribute, states being shown on line charts 


Data collected from Desktop that are different from immersive system:

\textbf{Interaction: mouse click, mouse hover, keyboard, button clicked, time selected, attribute...
valueMonitorTap, valueMonitorGaze, valueMonitorVoice, valuemonitorAttribute, valuemonitorTime, valuemonitorDeselect,
objPosition.x, objPosition.y, objPosition.z, (obj name)}

$x_{t1}$: interaction type -- \{gaze over, selection of region, selection of attribute, selection of time, none of the others\}

$x_{t2} ... x_{t4}$: object location

$x_{t5}$: object type -- \{country, line chart\}

$x_{t6} ... x_{t8}$: user location

$x_{t9} ... x_{t11}$: user orientation

$x_{t12} ... x_{t14}$: user Up direction (head rotation)

$x_{t15}$: hand status -- \{air tap start, air tap finish, air tap started, none of the others\}




%PlotThread: Creating Expressive Storyline Visualizations using Reinforcement Learning
%https://zjuidg.org/source/projects/plotthread/plotthread.pdf
%Trained model to enable new functions --
%``employ a mixed-initiative approach where both the agent and designers work on the same canvas to boost the collaborative design of storylines."


%https://provenance-survey.caleydo.org/
%Guo H., Gomez S., Ziemkiewicz C., Laidlaw D. (2016). A Case Study Using Visualization Interaction Logs and Insight Metrics to Understand How Analysts Arrive at Insights IEEE Transactions on Visualization and Computer Graphics, 22 (1): 51-60. doi:10.1109/TVCG.2015.2467613
%Cho I., Wesslen R., Karduni A., Santhanam S., Shaikh S., Dou W. (2017). The Anchoring Effect in Decision-Making with Visual Analytics 2017 IEEE Conference on Visual Analytics Science and Technology (VAST), 116-126. doi:10.1109/VAST.2017.8585665
%Characterizing Exploratory Visual Analysis: A Literature Review and Evaluation of Analytic Provenance in Tableau
Previous work showed that interaction provenance can be used to understand users, reveal important stages of exploration process / strategies.

%https://onlinelibrary.wiley.com/doi/abs/10.1111/cgf.13402
Constellations supports deriving summary insights about prior investigations and supports the exploration of new, unexplored regions in the dataset.

The user study compared their system with notebooks.


%https://ieeexplore.ieee.org/document/8017614
``we introduce the Berkeley Analysis and Storage Toolkit (BASTet), a novel framework for shareable and reproducible data analysis that supports standardized data and analysis interfaces, integrated data storage, data provenance, workflow management, and a broad set of integrated tools."

%https://ieeexplore.ieee.org/document/7192728
evaluation - In a study comparing Voyager to a manual visualization specification tool, we find that Voyager facilitates exploration of previously unseen data and leads to increased data variable coverage

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

